Approximately Gaussian Replicator Flows: Nonconvex Optimization as a Nash-Convergent Evolutionary Game

This work leverages tools from evolutionary game theory to solve unconstrained nonconvex optimization problems. Specifically, we lift such a problem to an optimization over probability measures, whose minimizers exactly correspond to the Nash equilibria of a particular population game. To algorithmically solve for such Nash equilibria, we introduce approximately Gaussian replicator flows (AGRFs) as a tractable alternative to simulating the corresponding infinite-dimensional replicator dynamics. Our proposed AGRF dynamics can be integrated using off-the-shelf ODE solvers when considering objectives with closed-form integrals against a Gaussian measure. We theoretically analyze AGRF dynamics by explicitly characterizing their trajectories and stability on quadratic objective functions, in addition to analyzing their descent properties. Our methods are supported by illustrative experiments on a range of canonical nonconvex optimization benchmark functions.

==> tex/diag.tex <==
\subsection{Diagonal Approximation}
\label{sec: diagonal}

The size of the covariance matrix $C(t)$ grows quadratically in the problem dimension $n$. It is thus interesting to consider the impact of restricting $C(t)$ to be diagonal for all time $t$, for the purposes of numerical efficiency. The following proposition bounds the distance between $C(t)$ and its diagonal approximation.

\begin{proposition}
	\label{prop: diagonal}
	Let $h\colon \Rn \to \R^{n\times n}$, let $m \colon [0,\infty) \to \Rn$, and consider $C\colon [0,\infty) \to \R^{n\times n}$ solving the ODE
	\begin{equation*}
		\dot{C}_{ij}(t) = \E_{x\sim \N(m(t),C(t))}[h_{ij}(x)].
	\end{equation*}
	Also consider the diagonal approximation $D\colon [0,\infty) \to \R^{n\times n}$ solving the ODE
	\begin{equation*}
		\dot{D}_{ij}(t) = \begin{aligned}
			\begin{cases}
				\E_{x\sim \N(m(t),D(t))}[h_{ij}(x)] & \text{if $i=j$}, \\
				0 & \text{otherwise},
			\end{cases}
		\end{aligned}
	\end{equation*}
	with $D(0)$ diagonal. It holds that $D(t)$ is diagonal for all $t \in [0,\infty)$. Furthermore, if $C(0) = D(0)$ and $C(t),D(t)$ are positive definite for all $t\in [0,\infty)$, then
	\begin{align*}
		\|D(t) - C(t)\|_F^2 \le{}&\Bigg(\sum_{i,j : i\ne j} \|h_{ij}\|_\infty^2 \Bigg) \\
		\times \exp&\Bigg( \frac{9}{4} \sum_{i=1}^n \|h_{ii}\|_\infty^2 \int_{[0,t]}\|D(\tau)^{-1}\|_F^2 d\tau\Bigg),
	\end{align*}
	for all $t\in [0,\infty)$.
\end{proposition}

\begin{proof}
	The fact that $D(t)$ is diagonal for all $t$ is obvious. Suppose that $C(0) = D(0)$. Then, for $i=j$,
	\begin{align*}
		&|D_{ij}(t) - C_{ij}(t)| \\
		&\; = \Bigg|\int_{[0,t]} \big(\E_{x\sim \N(m(\tau),D(\tau))}[h_{ij}(x)] \\
		&\qquad - \E_{x\sim \N(m(\tau),C(\tau))}[h_{ij}(x)]\big) d\tau \Bigg| \\
		&\; \le \int_{[0,t]} \left| \left<h_{ij},\N(m(\tau),D(\tau)) - \N(m(\tau),C(\tau))\right>\right|d\tau \\
		&\; \le \int_{[0,t]} \|h_{ij}\|_\infty \left\|\N(m(\tau),D(\tau)) - \N(m(\tau),C(\tau))\right\|_\TV d\tau \\
		&\; \le \frac{3}{2} \|h_{ij}\|_\infty \int_{[0,t]} \min\left\{1,\sqrt{\sum_{k=1}^n \lambda_k(\tau)^2} \right\} d\tau,
	\end{align*}
	where $\lambda_k(t)$ is the $k$th largest eigenvalue of $D(t)^{-1}C(t) - I_n$ for all $t\in\Rpl$, with the final inequality following from \citet[Theorem~1.1]{devroye2018total}. Since
	\begin{align*}
		\sum_{k=1}^n \lambda_k(t)^2 &= \|D(t)^{-1} C(t) - I_n\|_F^2 \\
		&\le \|D(t)^{-1}\|_F^2 \|C(t) - D(t)\|_F^2,
	\end{align*}
	we find that
	\begin{align*}
		&|D_{ij}(t) - C_{ij}(t)| \\
		&\;\le \frac{3}{2}\|h_{ij}\|_\infty \int_{[0,t]}\min\{1,\|D(\tau)^{-1}\|_F \|C(\tau) - D(\tau)\|_F\} d\tau \\
		&\;\le \frac{3}{2} \|h_{ij}\|_{\infty} \int_{[0,t]} \|D(\tau)^{-1}\|_F \|C(\tau) - D(\tau)\|_F d\tau.
	\end{align*}
	Thus, by Jensen's inequality,
	\begin{align*}
		&|D_{ij}(t) - C_{ij}(t)|^2 \\
		&\quad\le \frac{9}{4} \|h_{ij}\|_\infty^2 \int_{[0,t]} \|D(\tau)^{-1}\|_F^2 \|C(\tau) - D(\tau)\|_F^2 d\tau.
	\end{align*}
	For $i\ne j$,
	\begin{align*}
		|D_{ij}(t) - C_{ij}(t)| &= \left|\int_{[0,t]} \E_{x\sim \N(m(\tau),C(\tau))}[h_{ij}(x)] d\tau \right| \\
		&\le \int_{[0,t]} \left| \left<h_{ij},\N(m(\tau),C(\tau))\right>\right|d\tau \\
		&\le \int_{[0,t]} \|h_{ij}\|_\infty \left\| \N(m(\tau),C(\tau))\right\|_\TV d\tau \\
		&= \|h_{ij}\|_\infty.
	\end{align*}
	Thus,
	\begin{align*}
		&\|D(t) - C(t)\|_F^2 \le \sum_{i,j : i\ne j} \|h_{ij}\|_\infty^2 \\
		&\quad+ \frac{9}{4} \sum_{i=1}^n \|h_{ii}\|_\infty^2 \int_{[0,t]} \|D(\tau)^{-1}\|_F^2 \|C(\tau) - D(\tau)\|_F^2 d\tau.
	\end{align*}
	The result follows by applying Gr\"onwall's lemma.
	% Hence, by Gr\"onwall's lemma, we conclude that
	% \begin{equation*}
	% 	\|D(t) - C(t)\|_F^2 \le \left(\sum_{i,j : i\ne j} \|h_{ij}\|_\infty^2 \right)\exp\left( \frac{9}{4} \sum_{i=1}^n \|h_{ii}\|_\infty^2 \int_{[0,t]}\|D(\tau)^{-1}\|_F^2 d\tau\right).
	% \end{equation*}
\end{proof}

\hl{There are two key problems with \autoref{prop: diagonal}: 1) The $\|D(\tau)\|_F^2$ term goes to infinity as $\tau$ increases (assuming that indeed the diagonal matrix decreases towards the zero matrix, like we know the full covariance matrix does for quadratic optimization), and 2) The function $h$ should actually depend on $m(t)$ and $C(t)$; $h(x,m(t),C(t)) = (C - m(t)m(t)^\top)f(x) - x x^\top f(x) + m x^\top f(x) + x m^\top f(x)$ for the replicator dynamics. I believe the latter issue makes the bound invalid.}


==> tex/todo.tex <==
\section{To Do}
\label{sec: to_do}

Here is a running list of notes, ideas to explore, and to-do items.

\begin{enumerate}
	\item Current framing of our focus: No sampling (unlike other evolutionary methods), polynomial objectives (so that we can achieve no sampling).
	\item Intro structure: 1) General optimization with the kinds of problems we are trying to solve, 2) propagation of distribution-based algorithms, mention they are all sampling-based, which usually kills guarantees, 3) go into our insight into connections with evolutionary game theory, allowing for explicit dynamics equations that do not rely on log-likelihood sampling (since they are not in gradient flow form), 4) restrict down to polynomial focus.
	\begin{enumerate}
		\item Short primer on evolutionary games in the next (sub)section (problem statement?). Wait to define our explicit game that we consider to the proposed method section.
	\end{enumerate}
	\item Newton's method, which has quadratic convergence, falls into local minima (since it always defines a descent direction). On the other hand, past evolutionary methods can escape local minima, but either don't have guaranteed rates of convergence, or are linear (see CMA-ES). If ours achieves quadratic convergence and can escape local minima, this may be a great way of selling things.
	\begin{enumerate}
		\item Derive convergence rate of our method (which may be based on Newton's, since our flow approaches the Newton's flow as $t$ increases). Either give continuous-time convergence rate, or convergence rate of a discrete-time algorithm (e.g., with forward Euler).
	\end{enumerate}
	\item If we focus on polynomial optimization for closed-form integration, then we should remove our ``block box optimization'' framing of the problem.
	\begin{enumerate}
		\item If we focus on polynomial optimization, how do we motivate what we are doing if someone asks ``Why don't you just use moment-SOS heirarchies to get a global optimum?''
	\end{enumerate}
	\item Since we are using Gaussians to integrate against, it seems unnatural to enforce constraints (unlike measures with fixed support $X$). Therefore, we may need to remove the ``constrained optimization'' language and focus on unconstrained optimization (which is fine and still useful, think of machine learning).
	\item Future idea: Can we do local approximations of $f$ using sums of Gaussians? If so, we may still get closed-form integrals, but the magnitude of our approximations will die down at distances far from our search area. This may help us with stability when using large covariances, since we won't be integrating over regions of space with very large function values (like with polynomials). However, it may cause the method to move to fake or local minima if we aren't careful. Namely, the ``zero level'' should be higher than the function value of our starting mean and its minima, to ensure that we are not too inclined to immediately move to explore regions too far away from the current search area (unless maybe this is a good thing and we want it). If we use Gaussian approximations for our function, can we use FFT to compute the approximations very quickly?
	\item Give local convergence theory for our flows (Lyapunov for continuous time, then maybe connect to the discrete or claim ODE solver will handle for sufficiently well-behaved polynomials)
	\item Bound difference between approximate Gaussian replicator flows and the true replicator flows. If cts-time, Gronwall? Otherwise, look into discrete time as well.
	\item Does our method enjoy the ``invariance'' properties discussed in the NES and IGO papers?
	\item IGO paper uses natural gradient in the parameter space, making it parameter-invariant. Does our replicator dynamic method do this automatically?
	\item What is rate of convergence of quadratic flow mean $m(t)$ from \eqref{eq: quadratic_flow_mean} to $-\frac{1}{2}A^{-1}b$? Is it linear, like gradient descent?
	\item When we discuss quadratic Gaussian flows (in closed form), can we instead assume that $A$ is only PSD, to show that $m(t)$ approaches a pseudo-inverse solution to the convex quadratic optimization problem?
	\item Are ReLU networks Gaussian-integrable? At least two-layer networks?
\end{enumerate}

\vspace*{\baselineskip}

For Proposition 8 on diagonal approximation:
\begin{enumerate}
	\item Mention what $h$ is.
	\item Tighten the bound by getting rid of the inverse matrix, which blows up as the covariance goes to zero. This appears to be a problem at the sub-multiplicative step for the Frobenius norm.
	\item Generalize to different $m(t)$ between the distributions, or mention how to by appealing to that same paper with the total variation distance bounds on Gaussians.
	\item Can we derive tighter bounds for the quadratic case? Specifically, one idea is this: The covariance evolution in the quadratic case was shown to be something like $\dot{C}(t) = -C(t)C(t)^\top$ (check the literature and our derivations). If we set $\dot{D}_{ij}(t) = - (D(t)D(t)^\top)_{ij}$ for $i=j$ and $\dot{D}_{ij}(t) = 0$ for $i\ne j$, then does $D(t) = C(t)$ for all $t$? Or, can we get a more easy bound since our ODEs are not in terms of expectations anymore?
\end{enumerate}

